Automated machine learning for borehole resistivity measurements

Deep neural networks (DNNs) offer a real-time solution for the inversion of borehole resistivity measurements to approximate forward and inverse operators. It is possible to use extremely large DNNs to approximate the operators, but it demands a considerable training time. Moreover, evaluating the network after training also requires a significant amount of memory and processing power. In addition, we may overfit the model. In this work, we propose a scoring function that accounts for the accuracy and size of the DNNs compared to a reference DNN that provides a good approximation for the operators. Using this scoring function, we use DNN architecture search algorithms to obtain a quasi-optimal DNN smaller than the reference network; hence, it requires less computational effort during training and evaluation. The quasi-optimal DNN delivers comparable accuracy to the original large DNN.

==> results/forward_optimal/atten_1.tex <==
\begin{tikzpicture}
\node (image) at (0,0)
{\includegraphics[width=5cm]{./results/forward_optimal/atten_1.png}};
\node[rotate=0] (gt) at (0.0,-2) {Ground truth};
\node[rotate=90] (pd) at (-2.2,0) {Predicted value};
%\node[rotate=0] (gt) at (0.0,2) {zz (conventional)};
\end{tikzpicture}


==> results/forward_optimal/atten_2.tex <==
\begin{tikzpicture}
\node (image) at (0,0)
{\includegraphics[width=6cm]{./results/forward_optimal/atten_2.png}};
\node[rotate=0] (gt) at (0.0,-2) {Ground truth};
\node[rotate=90] (pd) at (-2.2,0) {Predicted value};
\node[rotate=0] (gt) at (0.0,2) {zz (conventional)};
\end{tikzpicture}


==> results/forward_optimal/atten_6.tex <==
\begin{tikzpicture}
\node (image) at (0,0)
{\includegraphics[width=8cm]{Figures/automatic_plots/Cross_plot_final/atten_Deep_xxyyzz_56.png}};
%\node[rotate=0] (I_h) at (0.0,2) {$d_u$};
\end{tikzpicture}


==> scoring_function/scoring_function.tex <==
\begin{tikzpicture}
\begin{axis}[
%  ymode=log,
%  xmode=log,
%  grid=both,
%  xmin=0,
%  ymin=0.0,
%  ymax=10,
%  height=.9*\textwidth,
%  width=0.7*\textwidth,
  height=6cm,
  width=5cm,
%  y=-0.5cm,
  y dir=reverse,
  xlabel={$h$},
  ylabel near ticks,
  ylabel={$R (h)$},  
]
\addplot [blue,line width=1.5,dashed] table [x = X,y = Y, dotted, mark=none]{scoring_function/scoring_function.odt};
\end{axis}
\end{tikzpicture}
%\caption{Analytical and numerically computed gradient}
%\label{fig_ex2_abs_field}
%\end{figure}

